Enhancing Training Data Attribution with Representational Optimization

Training data attribution (TDA) methods aim to measure how training data impacts a model's predictions. While gradient-based attribution methods, such as influence functions, offer theoretical grounding, their computational costs make them impractical for large-scale applications. Representation-based approaches are far more scalable, but typically rely on heuristic embeddings that are not optimized for attribution, limiting their fidelity. To address these challenges, we propose AirRep, a scalable, representation-based approach that closes this gap by learning task-specific and model-aligned representations optimized explicitly for TDA. AirRep introduces two key innovations: a trainable encoder tuned for attribution quality, and an attention-based pooling mechanism that enables accurate estimation of group-wise influence. We train AirRep using a ranking objective over automatically constructed training subsets labeled by their empirical effect on target predictions. Experiments on instruction-tuned LLMs demonstrate that AirRep achieves performance on par with state-of-the-art gradient-based approaches while being nearly two orders of magnitude more efficient at inference time. Further analysis highlights its robustness and generalization across tasks and models. Our code is available at https://github.com/sunnweiwei/AirRep

==> table/results.tex <==
\begin{table*}[t!]
    \centering\small
    \caption{LDS evaluation on FLAN. Averaged correlation score of all NLP tasks. \textit{Dim} refers to the dimensionality of the embeddings (equivalent to storage size), and \textit{Time Cost} indicates the seconds required to attribute 1,000 data points on a single A100 GPU.}
    \label{tab:all-flan}
    
    \begin{tabular}{l rccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Dim}} & \multirow{2}{*}{\textbf{Time Cost}} & \multicolumn{4}{c}{\textbf{Target Language Model}}  \\
& & & Qwen2.5-0.5B &  Qwen2.5-1.5B & Qwen2.5-3B & Qwen2.5-7B \\
% Repeat Training & - & - & 43.59 & - \\

% Repeat (TinyLlama) & - & 18.39 & \\
% Repeat (Instruct) & - & 36.54 & \\

\midrule
\textbf{Gradient-based methods} \\
\midrule
TracIn & 1152 & 96.3 & 4.21 & \\
TracIn & 768 & 96.3 & 4.21 & \\

\midrule

LESS-0.5B (proj 8196) & 8196 & 132.9 & 16.40	& 10.89	& 9.15	& 6.40 \\
LESS-0.5B (proj 768) & 768 & 132.9 & 10.67	& 7.04	& 5.55	& 4.23 \\

\hline

LESS-1.5B (proj 8196) & 8196 & 132.9 & - & 12.46 & 8.51	& 6.23 \\
LESS-1.5B (proj 768) & 768 & 132.9 & - & 7.35 & 5.48	& 3.66 \\

\hline

LESS-3B (proj 8196) & 8196 & 132.9 & - & - & 8.97	& 5.24 \\
LESS-3B (proj 768) & 768 & 132.9 & - & - & 4.81	& 3.17\\

\midrule
% Trak~\citep{Xia2024LESSSI} \\
LoGra-0.5B (rank=16)
 & 18432 & 33.10 &  19.75 & 12.94 & 10.13 & 7.96\\
LoGra-0.5B (rank=8)
 & 4608 &  33.42 & 16.22 &	10.86 &	8.41 & 6.86\\
LoGra-0.5B (rank=4)
 & 1152 & 33.84  & 13.32 & 8.84 & 6.72 & 6.26\\
 
 \hline
 LoGra-1.5B (rank=16)
 & 21504 & 66.64 &  - & \textbf{16.34}	& 11.37	& 8.38\\
LoGra-1.5B (rank=8)
 & 5376 &  66.64 & - & 13.34	& 9.78	& 7.93\\
LoGra-1.5B (rank=4)
 & 1344 & 66.64  & - & 10.58	& 7.43	& 6.53\\

\hline
LoGra-3B (rank=16)
 & 27648 & 104.96  & - & - & \textbf{13.38} & 8.75\\
LoGra-3B (rank=8)
 & 6912 &  104.96 & - & - & 10.97 &	7.69\\
 LoGra-3B (rank=4)
 & 1728 & 104.96 &  - & - & 8.39	& 6.12\\
 
\midrule
\textbf{Representation-based methods} \\
\midrule
TF-IDF & - & 0.40  & 2.52 & 1.63 & 3.11 & -0.15 \\
DSIR & - & 0.25 & 0.49 & 0.50 & -2.05 & -0.48 \\
\hline
RDS-0.5B (mean pooling) & \\
RDS-1.5B (mean pooling) & \\
RDS-3B (mean pooling) & \\
\hline
GTE (large) & 1024 & 2.54 & 1.62 & 2.05 & 0.62 & 4.06\\
GTE (base) & 768 & 1.13 & 1.49 & 1.81 & 1.43 & 0.58 \\
GTE (small) & 384 & 0.40 & 0.92 & 0.40 & 0.85	& 2.25 \\
% MATES & 768 & 1.98 & $1\times$ \\
% GTE-Base +Attention* & 768 & 1.28 & 2.74 & \textbf{26.78} & 7.96 & 36.18 \\
\midrule
\textbf{RepInf (Ours)} & 384 & 0.40 & \textbf{21.11}	& \underline{15.01} & \underline{12.31}	& \textbf{9.18} \\
% \midrule
% \textit{Ablation variants}\\
% (a) without attention pooling & 384 & 0.40 & 14.75 & 10.79 & 9.31 & 7.86 \\
% (b) without finetuned encoder \\
% (c) without loss weighting \\
% (d) with RMSE loss\\
\bottomrule
    \end{tabular}
\end{table*}

